Finitely Supported Sets Containing Infinite Uniformly Supported Subsets

The theory of finitely supported algebraic structures represents a reformulation of Zermelo-Fraenkel set theory in which every construction is finitely supported according to the action of a group of permutations of some basic elements named atoms. In this paper we study the properties of finitely supported sets that contain infinite uniformly supported subsets, as well as the properties of finitely supported sets that do not contain infinite uniformly supported subsets. For classical atomic sets, we study whether they contain or not infinite uniformly supported subsets.

==> eptcsdata.tex <==
\providecommand{\firstpage}{120}
\providecommand{\publicationstatus}{M. Marin, A. Cr\u{a}ciun (Eds.): \\
Working Formal Methods Symposium 2019 (FROM 2019)\\
EPTCS 303, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.303.9}{10.4204/EPTCS.303.9}}

